Discrete-time Negative Imaginary Systems from ZOH Sampling

A new definition of discrete-time negative imaginary (NI) systems is provided. This definition characterizes the dissipative property of a zero-order hold sampled continuous-time NI system. Under some assumptions, asymptotic stability can be guaranteed for the closed-loop interconnection of an NI system and an output strictly negative imaginary system, with one of them having a one step advance. In the case of linear systems, we also provide necessary and sufficient frequency-domain and LMI conditions under which the definition is satisfied. Also provided is a simple DC gain condition for the stability results in the linear case.

==> Conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
This paper investigates a state feedback stabilization problem using nonlinear NI systems theory for affine nonlinear systems with relative degree less than or equal to two. For such a system that also has a normal form, we provide a state feedback control law that makes it nonlinear NI or OSNI. In this case, if the internal dynamics of the system are ISS, then there exists state feedback control that stabilizes the system. In the case that the system has a nonlinear NI uncertainty, there exists a state feedback control law such that stabilizes the system if a positive definiteness-like assumption is satisfied for the storage function of the closed-loop system. A numerical example is provided to illustrate the process of stabilizing a system with a nonlinear NI uncertainty. Simulation shows that stabilization is achieved, as expected according to the proposed results.

==> Preliminaries.tex <==
\section{PRELIMINARIES}\label{sec:pre}
\begin{lemma}\label{lemma:DT_NI lemma}\cite{ferrante2017discrete}
Let $(A,B,C,D)$ be a minimal state-space realization of a discrete time, symmetric, real, rational, proper transfer function $G(z)$. Suppose $\det (I+A)\neq 0$ and $\det (I-A)\neq 0$. Then, $G(z)$ is NI if and only if there exists a real matrix $X=X^T>0$ such that
\begin{equation}\label{eq:DT_NI lemma}
X-A^TXA\geq 0 \quad \text{and}  \quad C=-B^T(A^T-I)^{-1}X(A+I).	
\end{equation}
\end{lemma}













